Speeding up Krylov subspace methods for computing f(A)b via randomization

This work is concerned with the computation of the action of a matrix function f(A), such as the matrix exponential or the matrix square root, on a vector b. For a general matrix A, this can be done by computing the compression of A onto a suitable Krylov subspace. Such compression is usually computed by forming an orthonormal basis of the Krylov subspace using the Arnoldi method. In this work, we propose to compute (non-orthonormal) bases in a faster way and to use a fast randomized algorithm for least-squares problems to compute the compression of A onto the Krylov subspace. We present some numerical examples which show that our algorithms can be faster than the standard Arnoldi method while achieving comparable accuracy.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Krylov subspace methods and randomization for $\lowercase{f}(A)\lowercase{b}$}{A. Cortinovis, D. Kressner, and Y. Nakatsukasa}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Speeding up Krylov subspace methods 
for computing {$\lowercase{f}(A)\lowercase{b}$} via randomization\thanks{Submitted to the editors DATE.
\funding{The work of AC has been partially supported by the SNSF research project \emph{Fast algorithms from low-rank updates}, grant number: 200020\_178806.}}}

% Authors: full names plus addresses.
\author{Alice Cortinovis\thanks{Department of Mathematics, Stanford University, Stanford, CA 94305, USA (\email{alicecor@stanford.edu}). } \and Daniel Kressner\thanks{Institute of Mathematics, EPFL, CH-1015 Lausanne, Switzerland (\email{daniel.kressner@epfl.ch}).} \and Yuji Nakatsukasa\thanks{Mathematical Institute, University of Oxford, Oxford, OX2 6GG, UK (\email{nakatsukasa@maths.ox.ac.uk}).}}
% \author{Dianne Doe\thanks{Imagination Corp., Chicago, IL 
%   (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
% \and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID 
%   (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
% \and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

